Transformed-Linear Innovations Algorithm for Modeling and Forecasting of Time Series Extremes

The innovations algorithm is a classical recursive forecasting algorithm used in time series analysis. We develop the innovations algorithm for a class of nonnegative regularly varying time series models constructed via transformed-linear arithmetic. In addition to providing the best linear predictor, the algorithm also enables us to estimate parameters of transformed-linear regularly-varying moving average (MA) models, thus providing a tool for modeling. We first construct an inner product space of transformed-linear combinations of nonnegative regularly-varying random variables and prove its link to a Hilbert space which allows us to employ the projection theorem, from which we develop the transformed-linear innovations algorithm. Turning our attention to the class of transformed linear MA($\infty$) models, we give results on parameter estimation and also show that this class of models is dense in the class of possible tail pairwise dependence functions (TPDFs). We also develop an extremes analogue of the classical Wold decomposition. Simulation study shows that our class of models captures tail dependence for the GARCH(1,1) model and a Markov time series model, both of which are outside our class of models.

==> references.tex <==
\begin{thebibliography}{xx}

\harvarditem{Bollerslev}{1986}{bollerslev1986}
Bollerslev, T.  \harvardyearleft 1986\harvardyearright , `Generalized
  autoregressive conditional heteroskedasticity', {\em Journal of Econometrics}
  {\bf 31},~307--327.

\harvarditem{Brockwell \harvardand\ Davis}{1991}{brockwelldavis1991}
Brockwell, P.~J. \harvardand\ Davis, R.~A.  \harvardyearleft
  1991\harvardyearright , {\em Time series: theory and methods}, Springer, New
  York.

\harvarditem{Cooley \harvardand\ Thibaud}{2019}{cooleythibaud2019}
Cooley, D. \harvardand\ Thibaud, E.  \harvardyearleft 2019\harvardyearright ,
  `Decompositions of dependence for high-dimensional extremes', {\em
  Biometrika} {\bf 106}(3),~587--604.

\harvarditem{Groetzner}{2020}{groetznerdur2020}
Groetzner, P. \&~D\"ur, M.  \harvardyearleft 2020\harvardyearright , `A
  factorization method for completely positive matrices', {\em Linear Algebra
  and its Applications} {\bf 591},~1--24.

\harvarditem{Hill}{1975}{hill1975}
Hill, B.~M.  \harvardyearleft 1975\harvardyearright , `A simple general
  approach to inference about the tail of a distribution', {\em The Annals of
  Statistics} {\bf 3},~1163--1174.

\harvarditem{Kiriliouk \harvardand\ Zhou}{2022}{kiriliouk2022}
Kiriliouk, A. \harvardand\ Zhou, C.  \harvardyearleft 2022\harvardyearright ,
  `Estimating probabilities of multivariate failure sets based on pairwise tail
  dependence coefficients'.

\harvarditem{Kulik \harvardand\ Soulier}{2020}{kuliksoulier2020}
Kulik, R. \harvardand\ Soulier, P.  \harvardyearleft 2020\harvardyearright ,
  {\em Heavy-tailed Time Series}, Springer-Verlag, New York.

\harvarditem{Lee}{2021}{leecooley2021}
Lee, J. \&~Cooley, D.  \harvardyearleft 2021\harvardyearright ,
  `Transformed-linear prediction for extremes', {\em arXiv preprint} .
\newline\harvardurl{arXiv:2111.03754v4}

\harvarditem{Mhatre}{2022}{mhatre2022}
Mhatre, N.  \harvardyearleft 2022\harvardyearright , Transformed-linear models
  for time series extremes, PhD thesis, Colorado State University.

\harvarditem{Mhatre \harvardand\ Cooley}{2020+}{mhatrecooley2020}
Mhatre, N. \harvardand\ Cooley, D.  \harvardyearleft 2020+\harvardyearright ,
  `Transformed-linear models for time series extremes', {\em arXiv Preprint} .
\newline\harvardurl{arXiv:2012.06705v3}

\harvarditem{Resnick}{2007}{resnick2007}
Resnick, S.~I.  \harvardyearleft 2007\harvardyearright , {\em Heavy-tail
  phenomena: probabilistic and statistical modeling}, Springer-Verlag, New
  York.

\harvarditem{Rudin}{1991}{rudin1991}
Rudin, W.  \harvardyearleft 1991\harvardyearright , {\em Functional analysis,
  2nd ed.}, McGraw-Hill, New York.

\harvarditem{Sargent}{1979}{sargent1979}
Sargent, T.~J.  \harvardyearleft 1979\harvardyearright , {\em Macroeconomic
  theory}, Economic theory, econometrics, and mathematical economics, Academic
  Press.

\harvarditem[Smith et~al.]{Smith, Tawn \harvardand\ Coles}{1997}{smithetal}
Smith, R.~L., Tawn, J. \harvardand\ Coles, S.  \harvardyearleft
  1997\harvardyearright , `Markov chain models for threshold exceedances', {\em
  Biometrika} {\bf 84},~249--268.

\end{thebibliography}

